Testing Density Discontinuity Using Spacings

In the regression discontinuity design, researchers assess the credibility of assumptions by testing the running variable's density for a discontinuity at the cutoff. This paper proposes a novel such test. The test uses q spacings on each side of the cutoff, where spacings are the widths between ordered observations. Spacings yield a continuous statistic that behaves well under weak assumptions. I study its properties in two asymptotic frameworks: one where q is fixed as the sample size increases and one where q slowly diverges to infinity. With q fixed, the test achieves exact asymptotic size control without user randomization. When q increases slowly, the test becomes consistent without sacrificing exact asymptotic size. Compared to the preferred version of Bugni and Canay's (2021) test, the only other test with comparably weak assumptions, this test reduces sensitivity to the tuning parameter and performs similarly when theirs is well-chosen.

==> jtload.tex <==
%% =====================================================================
%%  jtload.tex  --  journal-switching loader
%%
%%
%%     \def\JTjournal{qe}           % name of a file in jt/formats/ (no .jtf)
%%     \def\JTmode{submission}      % submission | final
%%     \def\JTpaperoptions{...}     % optional: paper-level key=value settings
%%
%%  Order of precedence for every setting (later wins):
%%     built-in defaults  <  journal format file  <  \JTpaperoptions
%% =====================================================================
\RequirePackage{keyval}
\makeatletter

%% ---------- mode ----------------------------------------------------
\providecommand\JTjournal{generic}
\providecommand\JTmode{submission}
\providecommand\JTpaperoptions{}
\providecommand\JTpart{main}               % main | supplement
\newif\ifJTfinal
\def\JT@tmp{final}\ifx\JTmode\JT@tmp \JTfinaltrue \fi
\newif\ifJTsupplement
\def\JT@tmp{supplement}\ifx\JTpart\JT@tmp \JTsupplementtrue \fi

%% ---------- settings (key = value) ---------------------------------
%% Every key stores its value in \JT@<key>. Defaults below = a plain
%% working-paper look. Format files and \JTpaperoptions override them.
\def\JT@defkey#1#2{%
  \@namedef{JT@#1}{#2}%
  \define@key{JT}{#1}{\@namedef{JT@#1}{##1}}}
\JT@defkey{class}{article}           % document class
\JT@defkey{classoptions}{}           % options passed to the class
\JT@defkey{fontsize}{12pt}           % 10pt|11pt|12pt|class
\JT@defkey{paper}{letterpaper}       % letterpaper|a4paper|class
\JT@defkey{margins}{1in}             % any length, a geometry option list in {...}, or class
\JT@defkey{spacing}{1.5}             % single|onehalf|double|<stretch factor>|class
\JT@defkey{font}{cm}                 % cm|times|palatino|libertine|class
\JT@defkey{titleblock}{plain}        % plain|titlepage|econsoc|elsarticle
\JT@defkey{refs}{beforeappendix}     % beforeappendix|end
\JT@defkey{refsname}{References}     % heading used for the reference list
\JT@defkey{bibstyle}{plainnat}       % .bst used with \JTbibtex
\JT@defkey{natbib}{authoryear}       % natbib options; "class" if the class loads natbib
\JT@defkey{floats}{intext}           % intext | ownpage (each float alone on a page, in text order) | end (endfloat)
\JT@defkey{floatmarkers}{true}       % floats=end: leave "[Table 1 about here.]" in the text
\JT@defkey{anonymous}{false}         % true = suppress authors, affiliations, thanks
\JT@defkey{linenumbers}{false}       % true|false|class
\JT@defkey{showjel}{true}            % print JEL codes on the title page
\JT@defkey{showkeywords}{true}
\JT@defkey{showdate}{true}
\JT@defkey{abstractwords}{0}         % warn if the abstract exceeds this (0 = no check)
\JT@defkey{maxlines}{0}              % warn if lines/page exceed this (0 = no check)
\JT@defkey{maxpages}{0}              % warn if the document exceeds this (0 = no check)
\JT@defkey{qedsymbol}{default}       % default|filled
\JT@defkey{thmstyle}{plain}          % amsthm style for theorem-like environments
\JT@defkey{thmcounter}{separate}     % separate|shared   (shared = Lemma 2.3 after Theorem 2.2)
\JT@defkey{thmwithin}{section}       % section|none
\JT@defkey{eqwithin}{none}           % section|none
\JT@defkey{appendixeq}{continue}     % letter = (A.1) in appendices | continue
\JT@defkey{appendixfloats}{letter}   % letter = Table A.1 in appendices | continue
\JT@defkey{theorems}{standard}       % standard | none (define your own)
\JT@defkey{externaldoc}{}            % aux file to read labels from (main <-> supplement)
\JT@defkey{twocolumn}{false}
\JT@defkey{eqshrink}{true}           % last resort: shrink displays that still overflow
\JT@defkey{eqminscale}{0.80}         % warn loudly below this scale
\JT@defkey{hyperref}{true}
\JT@defkey{linkcolor}{blue}          % blue|black (black for print-like output)
\JT@defkey{jelname}{JEL classification}
\JT@defkey{footnotespacing}{single}  % single | body (footnotes keep the body spacing)
\JT@defkey{defstyle}{definition}     % amsthm style for definitions (ET: plain = italic)
\JT@defkey{thanksplace}{footnote}    % footnote | section (acknowledgments section before the references)
\JT@defkey{declorder}{}              % sections before the references, in order: ack,funding,competing,ai
\JT@defkey{declomit}{}               % declarations not printed at all (e.g. JoE collects competing interests online)
\JT@defkey{ackname}{Acknowledgments}
\JT@defkey{fundingname}{Funding}
\JT@defkey{competingname}{Competing interests}
\JT@defkey{ainame}{Declaration of generative AI use}
\JT@defkey{minkeywords}{0}           % warn if fewer keywords (0 = no check)
\JT@defkey{maxkeywords}{0}           % warn if more keywords (0 = no check)
\JT@defkey{keywordsalpha}{false}     % warn unless keywords are in alphabetical order
\JT@defkey{keywordsnotintitle}{false}% warn if a keyword appears in the title
\JT@defkey{requirejel}{false}        % warn if \JTjel is empty
\JT@defkey{requireemail}{false}      % warn if the corresponding author has no e-mail
\JT@defkey{runningheadmax}{0}        % warn if \JTshorttitle is longer (0 = no check)
\JT@defkey{suppmaxpages}{0}          % page limit for supplement.tex (0 = no check)
\JT@defkey{pagesnote}{check what the limit counts}
\JT@defkey{keywordsname}{Keywords}
\JT@defkey{note}{}                   % free text shown in the log/summary (e.g. "VERIFY")
\newcommand\JTset[1]{\setkeys{JT}{#1}}

%% Hooks a format file may fill (see jt/formats/_NEW_JOURNAL.jtf):
\newcommand\JT@afterclass{}          % code run right after the class is loaded
\newcommand\JT@beginhook{}           % code run at \begin{document}
\newcommand\JTafterclass[1]{\g@addto@macro\JT@afterclass{#1}}
\newcommand\JTatbegindocument[1]{\g@addto@macro\JT@beginhook{#1}}
\newcommand\JT@appendixhook{}        % code run by \JTappendix after \appendix
\newcommand\JTatappendix[1]{\g@addto@macro\JT@appendixhook{#1}}

%% ---------- read the journal format, then paper overrides -----------
\input{\JTjournal.jtf}
\expandafter\JTset\expandafter{\JTpaperoptions}
%% options given on the command line (e.g. by tools/build-all.sh) win over all
\providecommand\JTextraoptions{}
\expandafter\JTset\expandafter{\JTextraoptions}

%% ---------- assemble class options and load the class ---------------
\def\JT@clsopts{}
\def\JT@addopt#1{\ifx\JT@clsopts\@empty\def\JT@clsopts{#1}\else
  \expandafter\def\expandafter\JT@clsopts\expandafter{\JT@clsopts,#1}\fi}
\def\JT@tmp{class}%
\edef\JT@x{\JT@fontsize}\ifx\JT@x\JT@tmp\else\expandafter\JT@addopt\expandafter{\JT@x}\fi
\edef\JT@x{\JT@paper}\ifx\JT@x\JT@tmp\else\expandafter\JT@addopt\expandafter{\JT@x}\fi
\def\JT@tmp{true}\edef\JT@x{\JT@twocolumn}\ifx\JT@x\JT@tmp\JT@addopt{twocolumn}\fi
\edef\JT@x{\JT@classoptions}\ifx\JT@x\@empty\else\expandafter\JT@addopt\expandafter{\JT@x}\fi
\typeout{jt: journal=\JTjournal, mode=\JTmode, class=\JT@class [\JT@clsopts]}
%% arXiv copy: main.tex loads the class itself.
\makeatletter
\JT@afterclass
\makeatother\usepackage{jtcore}

